A Methodology for Obtaining Objective Measurements of Population Obesogenic Behaviors in Relation to the Environment

The way we eat and what we eat, the way we move and the way we sleep significantly impact the risk of becoming obese. These aspects of behavior decompose into several personal behavioral elements including our food choices, eating place preferences, transportation choices, sleeping periods and duration etc. Most of these elements are highly correlated in a causal way with the conditions of our local urban, social, regulatory and economic environment. To this end, the H2020 project "BigO: Big Data Against Childhood Obesity" (http://bigoprogram.eu) aims to create new sources of evidence together with exploration tools, assisting the Public Health Authorities in their effort to tackle childhood obesity. In this paper, we present the technology-based methodology that has been developed in the context of BigO in order to: (a) objectively monitor a matrix of a population's obesogenic behavioral elements using commonly available wearable sensors (accelerometers, gyroscopes, GPS), embedded in smart phones and smart watches; (b) acquire information for the environment from open and online data sources; (c) provide aggregation mechanisms to correlate the population behaviors with the environmental characteristics; (d) ensure the privacy protection of the participating individuals; and (e) quantify the quality of the collected big data.

==> tables/behavioural_indicators.tex <==
\begin{table}[!t]
  \begin{minipage}{\textwidth}
  \caption{Indicative list of behavioural indicators}
  \renewcommand{\arraystretch}{1.1}
  \label{table:behavioural_indicators}
  \begin{tabularx}{\linewidth}{Xll}
  %% \begin{tabular}{lll}
    \toprule
    \textbf{Name} & \textbf{Units} & \textbf{Sensors}
      \footnote{\textbf{L}: Location-related sensors, such as GPS,
        magnetometer. Either on the mobile phone or in wristband/smartwatch,
        \textbf{A}: Activity-related indicators, such as accelerometer,
        gyroscope. Either on the mobile phone or in wristband/smartwatch, \textbf{P}:
        Smartphone camera, \textbf{U}: User self-reports
        %% \textbf{O}: Operating System 
        %% \textbf{E}: External sources (e.g. Google maps),
        %% \textbf{O}: Media monitoring reports
      } \\
    \midrule
    \textbf{Diet Indicators} & & \\
    Eating fast food & Occurence & L, P, U \\
    Fast-food eating frequency & Times/week & L, P, U \\
    Eating dinner outside of the home? & Occurence & L, P, U \\
    Eating at home & Occurence & L, P, U \\
    Food type & Categorical & U, P \\
    Meal type (breakfast, lunch, dinner, snack) & Categorical & L, P, U \\
    Meal frequency (e.g., breakfast) & Occurrence & U,P \\
    Soda or fizzy drinks & Occurrence & U,P \\
    Diet soda & Occurrence & U,P \\
    Juice & Occurrence & U,P \\
    Drinking water & Occurrence & U,P \\
    Drinking milk & Occurrence & U,P \\
    \midrule
    \textbf{Physical Activity Indicators} - Calculated at minute intervals\\ 
    Energy expenditure & MET\footnote{MET: Metabolic Equivalent of Task} & A \\
    Activity type & Categorical & A \\
    Activity intensity & Categorical & A \\
    Activity level & Categorical & A \\
    Activity counts\cite{TODO} & Counts/Minute & A\\
    \textbf{Physical Activity Indicators} - Calculated daily or weekly & & \\
    Walking/cycling to/from school & Times/week & A, L \\
    Minutes of active commute to school & Minutes/day & A, L \\
    Exercise frequency & Times/week & A \\
    Minutes of Sedentary behaviours after school & Minutes/day & A \\
    Distribution of physical activity at school & Minutes per activity & A \\
    Distribution of Physical activity after school & Minutes per activity & U, A \\
    %% Frequency of 10 min bouts of consecutive mod-vig & Times/week & A \\ REMOVE
    \midrule
    \textbf{Sleep Indicators}\\
    Hours of sleep per night & Hours & A \\
    Sleep/wake-up times per night & Timestamp & A \\
    Movement during sleep & Categorical & A \\
    \bottomrule
  \end{tabularx}
  \end{minipage}
\end{table}


==> tables/lecs_aggregate.tex <==
\begin{table}[!t]
  \begin{minipage}{\textwidth}
  \caption{LECs based on aggregate children statistics} 
  \renewcommand{\arraystretch}{1.1}
  \label{table:lecs_aggregate}
  \begin{tabularx}{\linewidth}{lX}
  %% \begin{tabular}{lll}
    \toprule
    \textbf{Name} & \textbf{Units} \\
    \midrule
    Number of children visited geohash\footnote{Geohashes are
      alphanumeric strings following a geocoding mechanism which
      defines a hierarchical grid of rectangular regions around the
      globe. Each geohash is a rectangular region. The longer the
      length of the geohash, the smaller the region. For more details,
      see also Section TODO.} or PoI & Number \\
    Number of meals registered at geohash or PoI & Number \\
    Average PA of children at geohash or PoI at specific time segments & METs \\
    Distribution of means of transportation for geohash or PoI & Frequency per transportation mode \\
    Most common path from (geohash or public PoI) A to B &
    Series of locations or geohashes defining the path \\
    \bottomrule
  \end{tabularx}
  \end{minipage}
\end{table}


==> tables/lecs_behaviour_combinations.tex <==
\begin{table}[!t]
  \begin{minipage}{\textwidth}
  \caption{Examples of individual-level measurements resulting from a
    combination of LECs and behaviour, without necessarily revealing
    the location of individuals} 
  \renewcommand{\arraystretch}{1.1}
  \label{table:lecs_behaviour_combination}
  \begin{tabularx}{\linewidth}{Xl}
  %% \begin{tabular}{lll}
    \toprule
    \textbf{Name} & \textbf{Units} \\
    \midrule
    Time spent in open spaces in neighbourhood & Minutes/week \\
    Number of times per week user is within 400 m of food outlet & Frequency \\
    Time spent in recreational facilities & Minutes/week \\
    Distance from school to home & Kilometres \\
    \bottomrule
  \end{tabularx}
  \end{minipage}
\end{table}


==> tables/raw_sensor_data.tex <==
\begin{table}[!t]
  \begin{minipage}{\textwidth}
  \caption{Recorded raw signal types}
  \renewcommand{\arraystretch}{1.5}
  \label{table:raw_sensor_data}
  \begin{tabularx}{\linewidth}{lXl}
    \toprule
    \textbf{Sensor} & \textbf{Description} & \textbf{Frequency} \\
    \midrule
    Accelerometer & 
    Measures the acceleration force (in $m/s^2$) that is applied to a device on all
    three physical axes ($x$, $y$, and $x$), including the force of
    gravity. & 
    \makecell[tl]{slow ($5$ - $25$ $Hz$) \\ fast ($50$ - $200$ $Hz$)} \\

    Barometer &
    Measures the ambient air pressure (in $hPa$ or $mbar$) &
    $5$ - $25$ $Hz$ \\

    Light & 
    Measures the ambient light level (in $lx$) &
    $\frac{1}{60}$ - $5 Hz$ \\

    Proximity & Measures the proximity of an object relative to the
    view screen of a device (in $cm$). This sensor is typically used
    to determine whether a handset is being held up to a person's
    ear. &
    \makecell[tl]{depends on user \\ ($< \frac{1}{60} Hz$)} \\

    Humidity &
    Measures the relative ambient humidity (in $\%$) &
    $1$ $Hz$ \\  

    Thermometer &
    Measures the ambient room temperature (in $\degree C$) &
    $1$ $Hz$\\

    GPS & Information acquired from each visited location, including
    longitude and latitude (degrees), altitude ($m$), bearing
    (degrees), accuracy ($m$) and the speed ($m/s$). &
    $\frac{1}{60} Hz$\\
    

    \bottomrule
  \end{tabularx}
  \end{minipage}
\end{table}    

